Building Efficient Query Engines in a High-Level Language

Abstraction without regret refers to the vision of using high-level programming languages for systems development without experiencing a negative impact on performance. A database system designed according to this vision offers both increased productivity and high performance, instead of sacrificing the former for the latter as is the case with existing, monolithic implementations that are hard to maintain and extend. In this article, we realize this vision in the domain of analytical query processing. We present LegoBase, a query engine written in the high-level language Scala. The key technique to regain efficiency is to apply generative programming: LegoBase performs source-to-source compilation and optimizes the entire query engine by converting the high-level Scala code to specialized, low-level C code. We show how generative programming allows to easily implement a wide spectrum of optimizations, such as introducing data partitioning or switching from a row to a column data layout, which are difficult to achieve with existing low-level query compilers that handle only queries. We demonstrate that sufficiently powerful abstractions are essential for dealing with the complexity of the optimization effort, shielding developers from compiler internals and decoupling individual optimizations from each other. We evaluate our approach with the TPC-H benchmark and show that: (a) With all optimizations enabled, LegoBase significantly outperforms a commercial database and an existing query compiler. (b) Programmers need to provide just a few hundred lines of high-level code for implementing the optimizations, instead of complicated low-level code that is required by existing query compilation approaches. (c) The compilation overhead is low compared to the overall execution time, thus making our approach usable in practice for compiling query engines.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
High-performance has always been the holy grail of database management systems. Traditional general-purpose 
compilers are not, however, trusted to sufficiently deliver on that front. Thus, a considerable aspect of the 
database developer's role is to act as a substitute (pre-)compiler, who is trusted to deliver fast code and who 
manually eliminates abstraction and indirection overheads existing in the DBMS code. To do so, the developer has 
to work his way through the highly complicated and largely monolithic design of existing database systems. 

Such monolithic implementations are mostly driven by the dictate of performance: there 
conceptually separate components such as the storage manager, query engine, concurrency control, and 
recovery subsystems are all blended together into a single giant monolithic component. In addition, 
alternative implementations of data-structures are manually inlined for performance, leading to a great 
deal of redundancy. Debugging, maintainance and further development of such large code bases is, thus,
a very difficult task~\cite{DBLP:journals/pvldb/LometTZ11,kochmanifesto}.

In addition, and as illustrated in Figure 1, query compilation -- a prominent technique to significantly
boost the performance of a database system -- further sacrifices productivity for performance.
In general, query compilation approaches perform source-to-source compilation\footnote{Typically 
from C/C++ -- with which the DBMS system is originally written -- to optimized C/LLVM code.}
in order to optimize away the overheads of traditional database abstractions like the Volcano operator 
model~\cite{Volcano}. However, existing solutions do so in \textit{one} direct macro expansion 
step, using low-level code templates. This introduces an additional level of complexity when coding database
optimizations for two reasons. First, providing low-level code templates -- essentially in stringified form --
makes it hard or impossible to automatically typecheck the code templates. Second, since the templates 
are directly emitted by the generator, developers have to deal with a number of low-level concerns which make 
templates very difficult to implement and get right. For example, when generating LLVM~\cite{llvm} code 
developers must handle register allocation themselves. Code maintainance definetely becomes more 
complicated in the presence of query compilation\footnote{
The System R team actually reported that complicated maintenance was one of the main reasons that query compilation was 
abandoned in favor of interpretation~\cite{systemR}.}.
\begin{figure}[t!]
\centering
\begin{tikzpicture}

\pgfplotsset{
    every axis/.append style={
        scale only axis,
        width=0.85\columnwidth,
        height=3.6cm,
        xtick={0,0.05,0.1},
    },
    /tikz/every picture/.append style={
        trim axis left,
        trim axis right,
    }
}

 \begin{axis}[
      axis lines=left, xtick=\empty, ytick=\empty,
      xmin=0.8, ymin=0.5,
      xmax=5, ymax=5,
      nodes near coords,
      every node near coord/.append style={
          font=\small,         
          align=left,
          xshift=1.3cm,
          yshift=0.1cm,
          text width=2.5cm},
      x label style={at={(axis description cs:0.5,-0.03)},anchor=north},
      y label style={at={(axis description cs:-0.01,.5)},anchor=south},
      %y post scale=0.7,
      font=\small,
		xlabel=Performance,
		ylabel=Productivity]
	\addplot+[
      only marks, mark=x, mark size=3,
      point meta=explicit symbolic, color=black] 
   coordinates {
      (4, 4) [\textbf{\systemname}]
      (4, 1) [Handwritten\\Query Plans]
      (3, 2) [Query\\Compilers]
      (2, 3) [Existing\\DBMSes]
      (1, 4) [DBMS in High-Level Language]
	};
	\end{axis}
\end{tikzpicture}
\caption{Comparison of the performance/productivity tradeoff for all approaches
presented in this \paper{}.}
\label{designtradeoffs}
\end{figure}

On the other hand, modern high-level programming languages offer a number of software features
such as modules, interfaces and object-orientation (classes, objects, encapsulation, etc.). 
These features generally allow the same functionality to be implemented with fewer lines of code (compared to 
low-level languages like C), leading to increased productivity for developers. In addition, high-level 
languages come with powerfull type systems and well-defined design patterns that allow programmers not only to 
create abstractions and protect them from leaking, but also to quickly define system modules that are truly 
reusable (even in contexts very different from the one these components were created for) and easily 
composable~\cite{odersky_scalable}.  Using high-level programming can, effectively, put an end to the monolithic 
nature of database systems, thus making their overall maintenance significantly easier.

Unfortunately the use of high-level programming languages for DBMS development, despite leading to a much 
increased productivity for programmers, comes at a cost: such languages significantly increase indirection, 
which in turn has a pronounced negative performance impact. For example, abstraction generally necessitates 
the need of containers, leading to a significant amount of object creation and destruction operations at runtime.
Encapsulation is provided through object copying rather than object referencing, a fact that introduces a number
of memory allocations on the critical path. Even primitive types such as integers are often converted to their object
counterparts for use with general-purposes libraries. 

The \textit{abstraction without regret} vision~\cite{koch,kochmanifesto} draws
inspiration from the recent use of high-level languages for complex system development (e.g.\ the Singularity Operating 
System~\cite{singularity}) to argue that it is now time for a radical rethinking of how database systems and their optimizations are designed: 
by colliding with the traditional wisdom which calls for the use of low-level languages like C for high-performance 
DBMS development and using high-level languages instead, it is indeed possible to build database management systems 
that allow for both productivity and high performance, instead of trading-off the former for the latter. By programming 
databases in a high-level style and still being able to get good performance, the time saved can be spent implementing 
more data\-base features and optimizations.

In this \paper{} we realise this vision on the domain of ad-hoc, analytical query processing. We present {\systemname}, 
an in-memory query execution engine written in the high-level programming language Scala, being the first step towards 
providing a full DBMS written in a high-level language. 

To avoid the overheads of a high-level language (e.g.\  
complicated memory management) while maintaining well-defined abstractions, we convert the high-level Scala code that 
constitutes the query engine to optimized, low-level C code for each incoming SQL query. 
We do so by using \emph{generative} programming~\cite{taha00staging}, a technique that allows for programmatic removal 
of abstraction overhead through source-to-source compilation. This is a key benefit as, in contrast to traditional, 
general-purpose compilers, which need to perform complicated and so\-metimes brittle analyses before (maybe) 
optimizing programs, generative programming in Scala takes advantage of the type system of the language 
to provide programmers with strong \textit{guarantees} about the structure
of the generated code. For example, developers can ensure that certain abstractions 
(e.g.\ generic \datastructures and function calls) are definitely optimized away during code generation. 

The combination of high-level and generative programming allows {\systemname} to extend the 
scope of compilation optimization and perform \textit{whole-program} optimization, by specializing all \datastructures 
and auxiliary functions used by a query. This design significantly contrasts our approach with existing query 
compilation approaches (e.g.\ the one proposed in~\cite{neumann11}) for two reasons. First, a compiler that only 
handles queries cannot optimize and inline their code {\em with} the remaining code of the database system (which is 
typically \textit{pre-compiled}), thus missing opportunities to further improve performance. Second, in their purest 
form, existing approaches simply optimize or inline the code of \textit{individual} operators in the physical query plan, 
thus making cross-operator code optimization inside the query compiler impossible.

This \paper{} makes the following three contributions:
\begin{itemize}
\addtolength{\itemsep}{1ex}
\item 
It presents the \systemname{} query engine, which is based on a \textit{new} optimizing compiler called \compilerdefined. 
Even though there exist compiler frameworks (e.g.~\lmsdefined~\cite{lms}) for applying generative programming in 
high-level languages like Scala, it is our observation that such approaches do not scale to large and complex code bases, 
for at least two reasons. 
\vspace{1ex}

First, high-level systems code will employ a hierarchy of components and libraries from relatively high to very 
low level of abstraction. Composing and optimizing these for maximum efficiency requires tight control on the 
compiler's phases -- admitting custom optimization phases and phase orderings. 
This is necessary as code transformers with different optimization roles may have to be inlined in every possible 
ordering, depending on architectural, data, or query characteristics. 
\vspace{1ex}

However, current optimizing compilers do not offer much control over the process. For example, \lms{} applies 
\textit{all} user-specified, domain-specific optimizations and performs code generation in a \textit{single} 
optimization step\footnote{
\lms{} argues that the design choice of applying multiple optimizations in the same optimization phase is necessary in 
order to avoid the well-known \textit{phase-ordering} problem in compilers, where applying two (or more) optimizations in 
an improper order can lead not only to suboptimal performance but also to semantically incorrect generated 
programs~\cite{tiark-phd-thesis}. We analyze how the design of the new optimizing compiler, \compiler, differs from that 
of \lms{} in Section~\ref{sec:system} of this \paper{}. 
}. 
The absence of control over the order of optimizations effectively pollutes the code-base of individual optimizations. 
This is because the generated code may depend on the order of application, thus making some of these optimizations 
dependent to other, possibly semantically independent, optimizations. In general, the code complexity grows exponentially 
with the number of supported transformations\footnote{
As an example, consider the case of a compiler that is to support only two optimizations: 1) data-layout optimizations 
(i.e.\ converting a row layout to a column or PAX-like layout~\cite{Ailamaki:2001:WRC:645927.672367}) and 2) data-
structure specialization (i.e.\ adapting the definition of a data structure to the particular context in which 
it is used). This means that if the second optimization handles 3 different types of specialization, one has to provision 
for $2 \times 3 = 6$ cases in order to handle all possible combinations of these optimizations.
}.
\vspace{1ex}

Second, existing optizing compilers expose a large number of low-level, compiler internals such as nodes of an 
intermediate representation (IR), dependency information encoded in IR nodes, and code generation templates to their 
users. This necessary interaction with low-level semantics when coding optimizations, but more importantly the 
introduction of the IR as additional level of abstraction significantly increases the difficulty of debugging as 
developers cannot easily track the relationship between the source code, the optimization for it, expressed using IR 
constructs, and the final, generated code~\cite{yinyang,forge}.
\vspace{1ex}

Instead, the \compiler compiler was designed from the beginning so that it allows developers to have full-control 
over the optimization process without exporting compiler internals such as 
code generation templates. It does so by delivering sufficiently powerful programming abstractions to developers
like those afforded by modern high-level programming languages. 
However, of more importance to this \paper{} is the fact
that \compiler by design (as explained later in Section~\ref{sec:system}) enforces the separation of concerns among 
different optimizations (by applying them in multiple, distinct optimization phases), thus making it easier to both detect and resolve elusive performance bottlenecks in the \systemname{} 
query engine. \compiler's native language is Scala, and the system as well as the compiler extensions are 
all written in \textit{plain} Scala, thus allowing developers to be highly-productive.

\item It provides an in-depth presentation of the list of optimizations supported by the \systemname{} query engine. 
While doing so, we also give a detailed presentation about the \textit{high-level} compiler interfaces that 
database developers need to interact with when coding optimizations, as well as a number of concrete code examples about how the 
implementation of our optimizations looks like in \compiler{}. We do so in order to demonstrate the expressive power and 
ease-of-use of the new \compiler compiler while optimizing system aspects and components that may differ significantly in structure and 
granularity of operations.
\vspace{1ex}

We also show that these optimizations are expressed as library components, thus providing a \textit{clean} separation from 
the base code of {\systemname} (e.g. that of query operators). This results in a number of nice design properties: 
optimizations are (a) adjustable to the characteristics of workloads and architectures, (b) configurable, so that they can
be turned on and off at demand and (c) composable, so that they can be easily chained but also so that higher-level 
optimizations can be built from lower-level ones. These properties are very hard to provide using existing compilation 
approaches. For each such optimization we present: (a) the \textit{domain-specific} conditions that need to be satisfied 
in order to apply it (if any) and (b) possible tradeoffs (e.g.\ improved execution time versus increased memory 
consumption). Finally, we examine which categories of database systems can benefit from applying each of our optimizations 
by providing a classification of the \systemname{} optimizations.

\item We perform an experimental evaluation in the domain of analytical query processing using the \tpch 
benchmark~\cite{tpch} and we show how both the tight control over the transformation pipeline as well as compiling with 
multiple optimization phases can lead to performance competitive to that of a standard, commercial in-memory database 
called \timesten and the code generated by the query compiler of the \hyper system~\cite{neumann11}. We demonstrate how 
our query compilation strategy incurs negligible overhead to query execution. In addition, we illustrate that these 
performance improvements do not require significant programming effort from developers as even complicated optimizations 
can be coded in \systemname{} with only a few hundred lines of code. Finally, we provide insights on the performance 
characteristics and tradeoffs of individual optimizations. We do so by comparing major architectural decisions as fairly 
as possible, using a shared codebase that only differs by the effect of a single optimization. 
\end{itemize}

%More importantly, it grants 
%great flexibility to developers so that they can easily choose and experiment with a number of choices 
%when building query engines.

\commentout{
Software specialization is becoming increasingly important for overcoming
performance issues in complex software systems~\cite{StonebrakerOneSize}. 
This is not surprising: As Dennard's law has failed~\cite{dennard-scale-fail}, 
sequential computing hardware is not getting faster any more, and we have to look 
for parallelization and specialization opportunities for continued performance growth 
in computers. 

In the context of database management systems, it has been noted that query engines do
not, to date, match the performance of handwritten code~\cite{monetdb-handwritten}. 
Thus, query compilation strategies have been proposed in order to optimize away 
the overheads of traditional database abstractions like the Volcano operator model~\cite{Volcano}.
To this end, multiple players have been releasing query compilers for their database systems -- 
examples include Microsoft's Hekaton, Cloudera Impala, and MemSQL.
In the academic context, interest in query compilation has been renewed since 2009\footnote{Query compilation 
has been with us since the dawn of the era of relational database systems: IBM's \mbox{System R}~\cite{systemR} 
employed compilation in its very first prototype, but this approach was quickly abandoned in favor of 
query {\em interpretation} --
subsequently the mainstream and textbook approach
for query execution for 40 years.} and continues to grow
\cite{mohan-compilation,sql-generation-zhao,DBLP:journals/pvldb/AhmadK09,ferry-2,DBLP:conf/pods/Koch10,krikellas,neumann11,koch,dbtoaster,DBLP:journals/corr/CrottyGDKCZ14,kochmanifesto,Nagel:2014:CGE:2732977.2732984,DBLP:journals/debu/ViglasBN14,spark-sql,crotty-udf-centric,goel-scalable-analytics}
%Note not sure if we can include an anonymized legobase reference here.

Despite the differences between the individual approaches, all compilation
frameworks generate \textit{on-the-fly} an \textit{optimized} query evaluation 
engine for each incoming SQL query.
More importantly, most existing query compilers 
are, to the best of our knowledge, {\em template expanders}\/ at heart. A template expander is a procedure that, 
simply speaking, generates \textit{low-level} code in \textit{one} direct macro expansion 
step. This means that, while a query interpreter immediately {\em calls}\/ the 
operator implementations listed in a query plan, the template expander 
first {\em inlines} the code of each operator, to obtain low-level code for the 
\textit{entire} plan. While inlining, the template expander may also apply  
specific optimizations to the code of each \textit{individual} operator, before calling the final program.
We identify three main problems with existing approaches:
\begin{minipage}{\textwidth}
\vspace{\topsep}
\begin{itemize}
\addtolength{\itemsep}{1ex}

\item
{\em Limited scope and missed optimization potential of query compilation}. A compiler that only handles queries cannot optimize and inline
their code {\em with} the remaining code of the database system (which is typically \textit{pre-compiled}), thus missing opportunities to further improve performance.
In addition, in its purest form, template expansion makes cross-operator code optimization inside the query compiler impossible, as it simply
{\em inlines} the operator code in the plan, as discussed previously.

\item
{\em Limited adaptivity}. Systems such as LLVM~\cite{llvm} provide support for runtime optimization and just-in-time compilation for low-level languages
like C, but key runtime optimizations (such as those known from adaptive query processing) are only possible given query plans 
or high(er)-level code that a system such as LLVM
%, which receives code from a query compiler, 
never gets to see. For instance, LLVM will not be able to reverse-engineer the code it receives to make effective use of selectivity information.

\item
{\em Template expansion is brittle and hard to implement}.
Providing low-level code templates -- essentially in stringified form -- makes it hard or
impossible to automatically typecheck the code templates. Moreover, since the templates 
are directly emitted by the generator, developers have to deal with a number of 
low-level concerns which make templates very difficult to implement 
and get right. For example, when generating LLVM code developers must
handle register allocation themselves.
\vspace{1ex}

More importantly, template expanders make it impractical to support a large range of sophisticated optimizations since 
multiple code transformers (with different optimization roles) may have to be inlined in all possible orderings (depending
for example on architectural, data, or query characteristics). This fact causes a code size explosion in compiler code bases. For example, 
consider a template expander that is to 
support two optimizations: 1) data-layout optimizations (i.e.\ converting a row layout to a column or PAX-like
layout~\cite{Ailamaki:2001:WRC:645927.672367}) and 2) data-structure specialization (i.e.\ adapting the definition 
of a data structure to the particular context in which 
it is used). This means that if the second optimization handles 3 different types of specialization, one has to create a template 
expander with $2 \times 3 = 6$ cases to handle all possible combinations of these optimizations. In general, the code complexity grows 
exponentially with the number of supported transformations.
\vspace{1ex}

The System R team reported that complicated maintenance was one of the main reasons that query compilation was abandoned in favor of interpretation~\cite{systemR}.
\end{itemize}
\vspace{\topsep}
\end{minipage}

To overcome these performance and productivity limitations, we argue that that it is now time for a 
radical rethinking of how database systems that employ query compilation are designed. 
%The {\systemname} system~\cite{legobase} argues that DBMSes and query compilers 
%should, in general, allow for \textit{both} productivity and high performance, \textit{instead} of
%trading-off the former for the latter. 
To date, a considerable aspect of the database developer's role is 
to act as a substitute \mbox{(pre-)compiler}, who is trusted to deliver fast code and who manually eliminates 
abstraction and indirection overheads, a task that is often very tedious given the low-level, complicated and 
largely monolithic nature of many DBMS components\footnote{
Such monolithic implementations are mostly driven by the dictate of performance: there conceptually separate 
components such as the storage manager, query engine, concurrency control, and recovery subsystems 
are all blended together into a single giant monolithic component. In addition, alternative implementations of 
\datastructures are manually inlined for performance, leading to a great deal of redundancy, which
contributes to the very large code bases and the difficulty of maintaining them~\cite{DBLP:journals/pvldb/LometTZ11,kochmanifesto}.}. 
In addition, and as illustrated in Figure~\ref{designtradeoffs}, query compilation further
sacrifices productivity for performance, as developers now have to deal with an additional 
level of complexity when coding database optimizations. 
Instead, we argue that developers should be able to program
DBMSes and their optimizations efficiently at a high-level of abstraction, without 
experiencing negative performance impact.
%Next, we give a brief overview of the \systemname system and its overall contributions.

In this \paper{} we realise this vision on the domain of ad-hoc, analytical query processing\footnote{This vision has been previously called \textit{abstraction without regret}~\cite{koch,lms,kochmanifesto} and draws inspiration from the recent use of high-level languages for complex system development (e.g.\ 
the Singularity Operating System~\cite{singularity}).}. We present {\systemname}, an in-memory query execution engine written in the high-level programming language Scala, 
being the first step towards providing a full DBMS written in a high-level language. This is in 
contrast to the traditional wisdom which calls for the use of low-level languages like C for high-performance DBMS development. 
By programming databases in a high-level style and still being able to get good performance, the time 
saved can be spent implementing more data\-base features and optimizations. In addition, high-level 
programming allows to quick\-ly define system modules that are truly reusable (even in contexts very 
different from the one these components were created for) and easily composable~\cite{odersky_scalable}, thus 
putting an end to the monolithic nature of current database systems. This 
property makes the overall maintenance of the system significantly easier. More importantly, it grants 
great flexibility to developers so that they can easily choose and experiment with a number of choices 
when building query engines.
\begin{figure}[t!]
\centering
\begin{tikzpicture}

\pgfplotsset{
    every axis/.append style={
        scale only axis,
        width=0.85\columnwidth,
        height=3.6cm,
        xtick={0,0.05,0.1},
    },
    /tikz/every picture/.append style={
        trim axis left,
        trim axis right,
    }
}

 \begin{axis}[
      axis lines=left, xtick=\empty, ytick=\empty,
      xmin=0.8, ymin=0.5,
      xmax=5, ymax=5,
      nodes near coords,
      every node near coord/.append style={
          font=\small,         
          align=left,
          xshift=1.3cm,
          yshift=0.1cm,
          text width=2.5cm},
      x label style={at={(axis description cs:0.5,-0.03)},anchor=north},
      y label style={at={(axis description cs:-0.01,.5)},anchor=south},
      %y post scale=0.7,
      font=\small,
		xlabel=Performance,
		ylabel=Productivity]
	\addplot+[
      only marks, mark=x, mark size=3,
      point meta=explicit symbolic, color=black] 
   coordinates {
      (4, 4) [\textbf{\systemname}]
      (4, 1) [Handwritten\\Query Plans]
      (3, 2) [Query\\Compilers]
      (2, 3) [Existing\\DBMSes]
      (1, 4) [DBMS in High-Level Language]
	};
	\end{axis}
\end{tikzpicture}
\caption{Comparison of the performance/productivity tradeoff for all approaches
presented in this \paper{}.}
\label{designtradeoffs}
\end{figure}
 
{\systemname} uses \emph{generative} programming~\cite{taha00staging} for DBMS development.
This approach provides two key benefits over existing query compilers: (a) programmatic 
removal of abstraction overhead and (b) applying optimizations on multiple stages. 

First, to avoid the overheads of a high-level language (e.g.\  complicated memory management) 
while maintaining well-defined abstractions, the Scala code that constitutes the {\systemname} 
query engine, despite its high-level appearance, is actually a source-to-source compiler that emits 
optimized, low-level C code for each incoming SQL query. In contrast to traditional compilers, 
which need to perform complicated and so\-metimes brittle analyses before (maybe) optimizing 
programs, generative programming in Scala takes advantage of the type system of the language 
in order to provide programmers with strong \textit{guarantees} about the shape and nature
of the generated code. For example, developers can ensure that certain abstractions 
(e.g.\ generic \datastructures and function calls) are definitely optimized away during code generation. 
%We demonstrate that generative programming can be used to optimize both traditional 
%pull-style (Volcano)~\cite{Volcano} and more recent push-style~\cite{Neumann11} query execution engines.

Second, generative programming allows optimization and {(re-)}\-compilation of code at various 
execution stages. This is a very important property, as it allows us to view databases as living
organisms.  When the system is first developed, high-level and non-optimal abstractions can be 
used to simplify the development process.  During deployment, as more information is gathered 
(e.g.\ runtime statistics, configuration and hardware specifications), we can \textit{continuously} 
``evolve'' the query engine by recompiling the necessary components in order to take advantage of 
up-to-date information. To our knowledge, {\systemname} is the first system to support such 
\textit{continuous runtime optimization} of the whole query engine. This design choice differentiates 
this system from query optimization frameworks such as Starburst~\cite{starburst}.

The combination of high-level and generative programming allows {\systemname} to extend (compared to existing query
compilation approaches like the one presented in~\cite{neumann11}) the scope of compilation and perform \textit{whole-program} 
optimization, by specializing all \datastructures and auxiliary functions used by a query. This is done by specifying custom, 
database-specific optimizations. These are implemented as library components, providing a \textit{clean} separation from the 
base code of {\systemname} (e.g. that of query operators). Optimizations are (a) adjustable to the characteristics of workloads and
architectures, (b) configurable, so that they can be turned on and off at demand and (c) 
composable, so that they can be easily chained but also so that higher-level optimizations can be built from 
lower-level ones. These properties are very 
hard to provide using existing template-based compilers. 

%This is the journal version of the {\legobase} paper. In addition to the contributions presented 
%in the original paper (as they were briefly highlighted above), we now make the following 
%three contributions: 
This \paper{} makes the following three contributions:
\begin{itemize}
\addtolength{\itemsep}{1ex}
\item 
It presents the \systemname{} query engine, which is based on a \textit{new} optimizing compiler called \compilerdefined. Even though there exist compiler frameworks (e.g.~\lmsdefined~\cite{lms}) for applying generative programming in high-level languages like Scala, it is our observation that 
%It offers a complete, \textit{from scratch}, re-implementation of the query engine presented in~\cite{legobase} %the original paper,
%using a different optimizing compiler called \compilerdefined. During development of the initial system, it became obvious 
%to us that 
%like \lmsdefined~\cite{lms} 
%(which was used in the %original implementation of~\cite{legobase}) 
such approaches do not scale to large and complex code bases, for at least two reasons. 
\vspace{1ex}

First, high-level systems code will employ a hierarchy of components and libraries from relatively high to very 
low level of abstraction. Composing and optimizing these for maximum efficiency requires tight control on the 
compiler's phases -- admitting custom optimization phases and phase orderings. This is not offered by current 
query compilers. For example, \lms{} applies \textit{all} user-specified, domain-specific optimizations and 
performs code generation in a \textit{single} optimization step, without providing users with much control 
over the process\footnote{
\lms{} argues that the design choice of applying multiple optimizations in the same optimization phase is necessary in order to avoid the well-known \textit{phase-ordering} problem in
compilers, where applying two (or more) optimizations in an improper order can lead not only to suboptimal performance 
but also to semantically incorrect generated programs~\cite{tiark-phd-thesis}. Note that this design choice does \textit{not} mean that \lms{} is a template expander. This is because \lms{} can effectively interleave multiple optimization and code-generation phases, one after another. Stated otherwise, \lms{} can iteratively apply the \textit{whole} set of domain-specific optimizations after each code generation phase. We analyze how the design of the new optimizing compiler, \compiler, differs from that 
of \lms{} in Section~\ref{sec:system} of this \paper{}. }. 
The absence of control over the order of optimizations effectively leads to, as was described above, a need for provisioning for 
all possible optimization orderings. This need severely limits current high-level query compilation frameworks, as optimizations become 
interdependent and the overall code-base quickly grows to unmanageable complexity. This pollutes the code-base 
of individual optimizations and may make some of them dependent to other, possibly semantically independent, optimizations.
\vspace{1ex}

Second, existing query compilers expose a large number of low-level, compiler internals such as nodes of an intermediate
representation (IR), dependency information encoded in IR nodes, and code generation templates to their users. This is true
even for frameworks like \lms{} that offer a high-level IR. This necessary interaction with low-level semantics when coding 
optimizations, but more importantly the introduction of the IR as additional level of abstraction significantly increases the difficulty
of debugging as developers cannot easily track the relationship between the source code, the optimization for it, expressed using IR constructs, 
and the final, generated code~\cite{yinyang,forge}.
\vspace{1ex}

Instead, the \compiler compiler was designed from the beginning so that it allows developers to have full-control 
over the optimization process without exporting compiler internals such as 
code generation templates. It does so by delivering sufficiently powerful programming abstractions to developers
like those afforded by modern high-level programming languages. 
However, of more importance to this \paper{} is the fact
that \compiler by design (as explained later in Section~\ref{sec:system}) enforces the separation of concerns among 
different optimizations (by applying them in multiple, distinct optimization phases), thus making it easier to both detect and resolve elusive performance bottlenecks in the \systemname{} 
query engine. \compiler's native language is Scala, and the system as well as the compiler extensions are 
all written in \textit{plain} Scala, thus allowing developers to be highly-productive.

\item It provides an in-depth presentation 
of the list of optimizations supported by the \systemname{} query engine. 
%More specifically, it presents
%a number of optimizations that were either (a) not previously described in the original paper (due to space constraints),
%or (b) not supported so far by the original \systemname{} system. 
For each such transformation we present: (a) 
the \textit{domain-specific} conditions that need to be satisfied in order 
to apply it (if any) and (b) possible tradeoffs (e.g.\ improved execution time versus increased memory consumption).
In addition, we 
%are now also able to 
provide more details about the \textit{high-level} compiler interfaces that 
database developers need  to interact with in \compiler{}, while we also present examples 
about how the implementation of our optimizations looks like in \compiler{}. We do so in order to 
demonstrate the expressive power and ease-of-use of the \compiler compiler.
Finally, we examine which categories of database systems can benefit from applying each of our optimizations by providing a classification of the \systemname{} optimizations.

\item 
%In the original paper 
%The authors have previously demonstrated in~\cite{legobase} that \lms{} 
%customized with transformations geared towards the domain of analytical queries can produce code 
%competitive to both a commercial in-memory database, called \timesten, and the query compiler of the 
%\hyper system~\cite{Neumann11} for the \tpch benchmark~\cite{tpch}. 
%In this \paper{}, 
We perform an experimental evaluation in the domain of analytical query processing using the \tpch benchmark~\cite{tpch} 
and we show how both the tight control over the transformation pipeline as well as compiling with multiple optimization phases can 
lead to performance competitive to that of a standard, commercial in-memory database called \timesten and the code generated
by the query compiler of the \hyper system~\cite{neumann11} (which uses template expansion).
We demonstrate how this compilation strategy incurs negligible overhead to query execution. 
In addition, we illustrate that these performance improvements do not require significant programming effort from developers as
even complicated optimizations can be coded in \systemname{} with only a few hundred lines of code.
%while the new system maintains the fast compilation times of the original {\legobase} query engine. 
Finally, we provide insights on the performance characteristics and tradeoffs of individual optimizations. We do so by comparing major architectural decisions as fairly as possible, using a shared codebase that only differs by the effect of a single optimization. 
\end{itemize}
}
\begin{figure}[t!]
\lstset{style=sqlstyle}
\centering

\pgfdeclarelayer{background}
\pgfsetlayers{background,main}

\begin{tikzpicture}[level/.style={sibling distance=2cm/#1, level distance=1.3cm}]

% Hidden node to ensure that figure 1 and 2 are of the same height
%\node[rectangle, minimum height=4.2cm, below, anchor=center] (placeholder) at (0, 0){};

\node[anchor=center, left] (note1){
\begin{lstlisting}
SELECT * FROM 
  (SELECT S.D,
    SUM(1-S.B) AS E,
    SUM(S.A*(1-S.B)),
    SUM(S.A*(1-S.B)*(1+S.C))
  FROM S 
  GROUP BY S.D) T, R
WHERE T.E=R.Z AND R.Q=3
\end{lstlisting}
};

\node (join) at (2.8, 1.3) {\ \ $\bowtie_{E = Z}$}
   child {node (proj) {$\Gamma_{D,aggs}$}      
      child {node (s) {$S$} [solid, ultra thick]} 
      [solid, ultra thick]
   }
   child {node (sel) {$\sigma_{Q=3}$} 
      child {node (r) {$R$} [ultra thick] }
      [ultra thick]
   };

\end{tikzpicture}

\caption{Motivating example showing missed optimizations opportunities by
existing query compilers that use template expansion.}
\label{fig:motivating_example}
\end{figure}

\noindent \textbf{Motivating Example.} To better understand the differences of
our work with previous approaches, consider the SQL query shown in
Figure~\ref{fig:motivating_example}.  This query first calculates some
aggregations from relation \textit{S} in the \groupby operator $\Gamma$.  Then,
it joins these aggregations with relation \textit{R}, the tuples of which are
filtered by the value of column \textit{Q}.  The results are then returned to
the user. Careful examination of the execution plan of this query, shown in the
same figure, reveals the following three basic optimization opportunities missed
by existing query compilers that use template expansion:
\begin{itemize}
\addtolength{\itemsep}{1ex}
\item First, the limited scope of existing approaches usually results in
performing the evaluation of aggregations in \textit{pre-compiled} DBMS code. Thus, each
aggregation is evaluated \textit{consecutively} and, as a result, common
sub-expression elimination cannot be performed in this case (e.g.\ in the
calculation of expressions \code{1-S.B} and \code{S.A*(1-S.B)}). This shows that,
if we include the evaluation of all aggregations in the \textit{compiled} final
code, we can get additional performance improvement. This motivates us to
extend the scope of compilation in this work.

\item Second, template-based approaches may result in unnecessary computation. 
This is because operators are not aware of each other. 
In this example, the
generated code includes two materialization points: (a) at the \groupby and (b)
when materializing the left side of the join. However, there is no need to
materialize the tuples of the aggregation in two different \datastructures as
the aggregations can be immediately materialized in the \datastructure of the
join.  Such \textit{inter-operator} optimizations are hard to express using
\textit{template-based} compilers. By high-level programming we can instead
easily pattern match on the operators, as we show in
Section~\ref{subsec:eliminate_materializations}.
 
\item Finally, the \datastructures have to be \textit{generic} enough for all
queries. As such, they incur significant abstraction overhead, especially when
these structures are accessed millions of times during query evaluation. Current
query compilers cannot optimize the \datastructures since these belong to the
pre-compiled part of the DBMS. Our approach eliminates these overheads as it
performs \textit{whole-program} optimization and compiles, along with the
operators, the \datastructures employed by a query. This
significantly contrasts our approach with previous work.  
\end{itemize}

The rest of this \paper{} is organized as follows. Section~\ref{sec:system}
presents the overall design of {\systemname}, along with a
detailed description of the APIs provided by the new \compiler{} optimizing compiler. 
Section~\ref{sec:optimizations} gives an in-depth presentation of all supported
compiler optimizations of our system in
multiple domains.
%along with a classification of these optimizations according to which category of database systems each one targets optimizing. 
Section~\ref{sec:eval} presents our evaluation, where we
experimentally show that our approach using the \compiler{} optimizing compiler can lead to significant 
benefits compared to (i) a commercial database system that does not employ query compilation and 
(ii) a database system that uses a template expander for query compilation.
%, and,
%finally, (iii) a query engine implemented using the \lms{} optimizing compiler.
% --> Note: cite original (anonymized paper here?)
%the original \systemname{} query engine implemented using the \lms{} compiler~\cite{legobase}. 
We also give insights about 
the memory footprint, data loading time and programming effort required when working with the \systemname{} system. 
%We also show how these performance improvements come at the cost of increased memory footprint but that they require 
%low compilation times and small programming effort. 
Section~\ref{sec:related} presents related work in compilation and compares our
approach with existing query compilers and engines. Finally,
Section~\ref{sec:conclusions} concludes. 
